Domain Alignment Meets Fully Test-Time Adaptation

A foundational requirement of a deployed ML model is to generalize to data drawn from a testing distribution that is different from training. A popular solution to this problem is to adapt a pre-trained model to novel domains using only unlabeled data. In this paper, we focus on a challenging variant of this problem, where access to the original source data is restricted. While fully test-time adaptation (FTTA) and unsupervised domain adaptation (UDA) are closely related, the advances in UDA are not readily applicable to TTA, since most UDA methods require access to the source data. Hence, we propose a new approach, CATTAn, that bridges UDA and FTTA, by relaxing the need to access entire source data, through a novel deep subspace alignment strategy. With a minimal overhead of storing the subspace basis set for the source data, CATTAn enables unsupervised alignment between source and target data during adaptation. Through extensive experimental evaluation on multiple 2D and 3D vision benchmarks (ImageNet-C, Office-31, OfficeHome, DomainNet, PointDA-10) and model architectures, we demonstrate significant gains in FTTA performance. Furthermore, we make a number of crucial findings on the utility of the alignment objective even with inherently robust models, pre-trained ViT representations and under low sample availability in the target domain.

==> related_work.tex <==
\section{Related Work}
In this section, we relate \name to literature on adaptation, feature modulation and alignment methods.\\
\noindent\textbf{Unsupervised domain adaptation:}
Unsupervised domain adaptation (UDA) has been an important problem of research in multiple application areas and in the past decade a plethora of solutions have been developed.
Broad classes of uda methods can be understood through the foundational work of Ben David \etal ~\cite{Ben-David:2010:TLD:1745449.1745461}, which provides an upper bound on error on target data that can be achieved using a hypothesis $h$ as the combination of three terms - namely the error on source data, the discrepancy between the source-target domains measured through $\mathcal{H}$-divergence, and lastly a term that measures the optimal error achievable in both the domains (often assumed to be negligible). 
Earlier works\cite{Saenko2010AdaptingVC,Gong2012GeodesicFK,pan2010domain,sun2017correlation,Subspace_alignment,sun2015subspace} also commonly referred to as shallow UDA methods mainly focused on minimizing statistical divergence between source and target features computed using hand-crafted feature methods such as SURF descriptors. 
More recent approaches however use powerful feature extractors such as convolutional neural networks (CNNs), and aim to jointly minimize source error along with domain divergence error. Adversarial learning~\cite{cite:NIPS14GAN} has been the workhorse in these solutions, and can be implemented with different additional regularizers~\cite{cite:JMLR16RevGrad,CDANLong,CYCADA, UNIT,cite:CVPR17pix2pix}. Additionally some recent works have considered the use of pseudo-labeling and self-training~\cite{saito2017asymmetric,zou2019confidence,shot}, on top of these regularization strategies to further boost the UDA performance. While this work focuses on investigating the efficacy of subspace alignment in matching complex feature distributions, it is straightforward to extend our approach with additional regularizers or self-training protocols.





\noindent\paragraph{Subspace based adaptation:}
\noindent\paragraph{Test-time adaptation:}





==> tables/source_recovery.tex <==
\begin{table}[t]
\begin{tabular}{|c|c|}
\hline
\rowcolor[HTML]{EBEBEB} 
Method    & Source Accuracy (\%) \\ \hline
\ptent     & 95.70           \\ \hline
\name    & 90.68           \\ \hline
\name-SD & 95.68           \\ \hline
\hline
Source Only & 97.2\\\hline
\end{tabular}
\end{table}
